Parametric multi-fidelity Monte Carlo estimation with applications to extremes

In a multi-fidelity setting, data are available from two sources, high- and low-fidelity. Low-fidelity data has larger size and can be leveraged to make more efficient inference about quantities of interest, e.g. the mean, for high-fidelity variables. In this work, such multi-fidelity setting is studied when the goal is to fit more efficiently a parametric model to high-fidelity data. Three multi-fidelity parameter estimation methods are considered, joint maximum likelihood, (multi-fidelity) moment estimation and (multi-fidelity) marginal maximum likelihood, and are illustrated on several parametric models, with the focus on parametric families used in extreme value analysis. An application is also provided concerning quantification of occurrences of extreme ship motions generated by two computer codes of varying fidelity.

==> command.tex <==
% =====================================
% PACKAGES
% =====================================
\RequirePackage[capitalize,nameinlink]{cleveref}[0.19]
\usepackage{enumitem}
\usepackage[title]{appendix}

% =====================================
% THEOREM ENVIRONMENTS
% =====================================
 \newtheorem{theorem}{\bf Theorem}[section]
 \newtheorem{lemma}{\bf Lemma}[section]
 \newtheorem{fact}{\bf Fact}[section]
 \newtheorem{corollary}{\bf Corollary}[section]
 \newtheorem{axiom}{\bf Axiom}[section]
 \newtheorem{condition}{\bf Condition}[section]
 \newtheorem{property}{\bf Property}[section]
 \newtheorem{proposition}{\bf Proposition}[section]
 % The next structures are like theorems, but not italicized, with an
 % empty box at the end.
 % (the empty box has been taken away. M. Taqqu)
 \newtheorem{@definition}{\bf Definition}[section]
 \newenvironment{definition}{\begin{@definition}\rm}{\end{@definition}}

\newtheorem{@example}{\bf Example}[section]
\newenvironment{example}{\begin{@example}\rm}{\end{@example}}
\crefname{@example}{Example}{Examples}

\newtheorem{@nonexample}{\bf (Non)Example}[section]
\newenvironment{nonexample}{\begin{@nonexample}\rm}{\end{@nonexample}}

\newtheorem{@remark}{\bf Remark}[section]
\newenvironment{remark}{\begin{@remark}\rm}{\end{@remark}}


% =====================================
% MATH OPERATORS
% =====================================
\newcommand {\cov}{\qopname\relax n{\textrm{Cov}}}
\newcommand {\var}{\qopname\relax n{\textrm{Var}}}
\newcommand {\vrb}{\qopname\relax n{\textrm{Vrb}}}
\newcommand {\corr}{\qopname\relax n{\textrm{Corr}}}


% =====================================
% BLACKBOARD BOLD SYMBOLS
% =====================================
\newcommand{\bbE}{\mathbb {E}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbone}{\mathbb{I}}
\newcommand{\bbN}{{\Bbb N}}
\newcommand{\bbZ}{{\Bbb Z}}
\newcommand{\bbC}{{\Bbb C}}
\newcommand{\bbQ}{{\Bbb Q}}
\newcommand{\bbF}{{\Bbb F}}
\newcommand{\bbL}{{\Bbb L}}
\newcommand{\bbB}{{\Bbb B}}
\newcommand{\bbX}{{\Bbb X}}
\newcommand{\bbY}{{\Bbb Y}}
\newcommand{\bbV}{{\Bbb V}}
\newcommand{\bbW}{{\Bbb W}}

% Alternative notations for expectation
\newcommand{\rE}{\textrm{E}}

% CALLIGRAPHIC SYMBOLS
\newcommand{\calN}{{\mathcal N}}
\newcommand{\calW}{{\mathcal W}}

% =====================================
% BOLD SYMBOLS (VECTORS AND MATRICES)
% =====================================
% Bold lowercase letters
\newcommand{\bfc}{{\boldsymbol c}}
\newcommand{\bfd}{{\boldsymbol d}}
\newcommand{\bfe}{{\boldsymbol e}}
\newcommand{\bfg}{{\boldsymbol g}}
\newcommand{\bfh}{{\boldsymbol h}}
\newcommand{\bfs}{{\boldsymbol s}}
\newcommand{\bfv}{{\boldsymbol v}}
\newcommand{\bfy}{{\boldsymbol y}}
\newcommand{\bfz}{{\boldsymbol z}}
% Bold uppercase letters
\newcommand{\bfA}{{\boldsymbol A}}
\newcommand{\bfB}{{\boldsymbol B}}
\newcommand{\bfC}{{\boldsymbol C}}
\newcommand{\bfG}{{\boldsymbol G}}
\newcommand{\bfI}{{\boldsymbol I}}
\newcommand{\bfN}{{\boldsymbol N}}
\newcommand{\bfR}{{\boldsymbol R}}
\newcommand{\bfS}{{\boldsymbol S}}
\newcommand{\bfT}{{\boldsymbol T}}
\newcommand{\bfU}{{\boldsymbol U}}
\newcommand{\bfV}{{\boldsymbol V}}
\newcommand{\bfW}{{\boldsymbol W}}
\newcommand{\bfX}{{\boldsymbol X}}
\newcommand{\bfY}{{\boldsymbol Y}}
\newcommand{\bfZ}{{\boldsymbol Z}}
\newcommand{\BYn}{\Bar \bfY_{1:n}}
\newcommand{\BYm}{\Bar \bfY_{n+1:n+m}}
\newcommand{\BYnm}{\Bar \bfY_{1:n+m}}

% Bold Greek letters
\newcommand{\btheta}{{\boldsymbol \theta}}
\newcommand{\bfgamma}{{\boldsymbol \gamma}}
\newcommand{\bmu}{{\boldsymbol \mu}}
\newcommand{\bSigma}{{\boldsymbol \Sigma}}
\newcommand{\bphi}{{\boldsymbol \phi}}
\newcommand{\balpha}{{\boldsymbol \alpha}}
\newcommand{\bbeta}{{\boldsymbol \beta}}
\newcommand{\bfeta}{{\boldsymbol \eta}}
\newcommand{\htheta}{\widehat{\btheta}}

% CONVERGENCE AND DISTRIBUTION SYMBOLS
\newcommand{\ind}{\overset{d}{=}}
\newcommand{\inD}{\overset{\mathcal{D}}{\rightarrow}}
\newcommand{\tod}{\overset{d}{\rightarrow}}
\newcommand{\topp}{\overset{p}{\rightarrow}}
\newcommand{\fdd}{\overset{fdd}{\longrightarrow}}

\newcommand {\D}[1]{\dot{#1}}
\newcommand {\indf}[1]{{1}_{\{#1 \}}}
\newcommand{\abs}[1]{\left\vert#1\right\vert}

% Bar notation
\newcommand{\fbar}{\overline{F}}
\newcommand{\xbar}{\overline{X}}
\newcommand{\ybar}{\overline{Y}}

% Hat notation (estimators)
\newcommand{\khat}{\what{k}}
\newcommand{\that}{\what{\tau}}
\newcommand{\xhat}{\what{X}}
\newcommand{\yhat}{\what{Y}}
\newcommand{\Rhat}{\what{R}}
\newcommand{\hmu}{\widehat{\mu}}
\newcommand{\hrho}{\widehat{\rho}}
\newcommand{\hSig}{\widehat \bSigma}

\newcommand {\revd}{\widetilde{d}}
\newcommand {\revb}{\widetilde{b}}
\newcommand {\revx}{\widetilde{X}}
\newcommand {\xn}{\{ X_n \}}


\newcommand {\argmin}[1]{\underset{#1}{\rm{argmin}}}
\newcommand {\argmax}[1]{\underset{#1}{\rm{argmax}}}
\newcommand {\argsup}[1]{\underset{#1}{\rm{argsup}}}

\newcommand {\pc}[1]{ #1^{\scriptsize pc}  }
\newcommand{\mf}{{\scriptsize mf}}

% =====================================
% MULTI-FIDELITY SPECIFIC NOTATION
% =====================================
\newcommand{\yhifi}{Y^{(1)}}
\newcommand{\ylofi}{Y^{(2)}}
\newcommand{\yjifi}{Y^{(j)}}
\newcommand{\yjoint}{(\yhifi, \ylofi)}
\newcommand{\ylofik}{Y^{(K+1)}}

\newcommand{\zhifi}{Z^{(1)}}
\newcommand{\zlofi}{Z^{(2)}}
\newcommand{\bzhifi}{\bfZ^{(1)}}
\newcommand{\bzlofi}{\bfZ^{(2)}}

\newcommand{\hhifi}{h^{(1)}}
\newcommand{\hlofi}{h^{(2)}}
\newcommand{\bhhifi}{\bfh^{(1)}}
\newcommand{\bhlofi}{\bfh^{(2)}}

\newcommand{\thifi}{\btheta^{(1)}}
\newcommand{\tlofi}{\btheta^{(2)}}

\newcommand{\Fhifi}{F^{(1)}}
\newcommand{\Flofi}{F^{(2)}}

\newcommand{\dhifi}{\yhifi_{1}, \dots, \yhifi_{n}}

% True parameters
\newcommand{\tstarh}{\btheta_{1}^\ast}
\newcommand{\tstarl}{\btheta_{2}^\ast}
\newcommand{\mustarh}{\mu_{1}^\ast}
\newcommand{\mustarl}{\mu_{2}^\ast}
\newcommand{\sigstarh}{\sigma_{1}^\ast}
\newcommand{\sigstarl}{\sigma_{2}^\ast}
\newcommand{\rhostar}{\rho^\ast}
\newcommand{\Iinvh}{I_{\btheta^\ast_1}^{-1}}
\newcommand{\Iinvl}{I_{\btheta^\ast_2}^{-1}}
\newcommand{\bIinvh}{\bfI_{\btheta^\ast_1}^{-1}}
\newcommand{\bIinvl}{\bfI_{\btheta^\ast_2}^{-1}}

% Parameters
\newcommand{\tone}{\btheta_1}
\newcommand{\ttwo}{\btheta_2}
\newcommand{\tot}{\btheta_{1,2}}

% Log-likelihood derivatives
\newcommand{\dl}{\dot{\ell}}
\newcommand{\ddl}{\Ddot{\ell}}

% Sample means for Y
\newcommand{\ybaro}{(\overline{Y^{(1)}})_{n}}
\newcommand{\ybarto}{(\overline{Y^{(2)}})_{n}}
\newcommand{\ybartm}{(\overline{Y^{(2)}})_{m}}
\newcommand{\ybart}{(\overline{Y^{(2)}})_{n+m}}

% Sample means for h(Y)
\newcommand{\hbaro}{\overline{h(Y^{(1)})}_{n}}
\newcommand{\hbarto}{\overline{h(Y^{(2)})}_{n}}
\newcommand{\hbartm}{\overline{h(Y^{(2)})}_{m}}
\newcommand{\hbart}{\overline{h(Y^{(2)})}_{n+m}}
\newcommand{\bhbaro}{\overline{\bfh(Y^{(1)})}_{n}}
\newcommand{\bhbarto}{\overline{\bfh(Y^{(2)})}_{n}}
\newcommand{\bhbartm}{\overline{\bfh(Y^{(2)})}_{m}}
\newcommand{\bhbart}{\overline{\bfh(Y^{(2)})}_{n+m}}

% Sample means for h^(j)(Y)
\newcommand{\hobaro}{\overline{h^{(1)}(Y^{(1)})}_{n}}
\newcommand{\htbarto}{\overline{h^{(2)}(Y^{(2)})}_{n}}
\newcommand{\htbartm}{\overline{h^{(2)}(Y^{(2)})}_{m}}
\newcommand{\htbart}{\overline{h^{(2)}(Y^{(2)})}_{n+m}}
\newcommand{\bhobaro}{\overline{\bfh^{(1)}(Y^{(1)})}_{n}}
\newcommand{\bhtbarto}{\overline{\bfh^{(2)}(Y^{(2)})}_{n}}
\newcommand{\bhtbartm}{\overline{\bfh^{(2)}(Y^{(2)})}_{m}}
\newcommand{\bhtbart}{\overline{\bfh^{(2)}(Y^{(2)})}_{n+m}}

% Sample means for Z
\newcommand{\zbaro}{(\overline{Z_l^{(1)}})_{n}}
\newcommand{\zbarto}{(\overline{Z_l^{(2)}})_{n}}
\newcommand{\zbartm}{(\overline{Z_l^{(2)}})_{m}}
\newcommand{\zbart}{(\overline{Z_l^{(2)}})_{n+m}}

% Sample means for Z_1 and Z_2
\newcommand{\zbaroone}{(\overline{Z_1^{(1)}})_{n}}
\newcommand{\zbartoone}{(\overline{Z_1^{(2)}})_{n}}
\newcommand{\zbartone}{(\overline{Z_1^{(2)}})_{n+m}}
\newcommand{\zbarotwo}{(\overline{Z_2^{(1)}})_{n}}
\newcommand{\zbartotwo}{(\overline{Z_2^{(2)}})_{n}}
\newcommand{\zbarttwo}{(\overline{Z_2^{(2)}})_{n+m}}

% Expectations
\newcommand{\Eho}{\bbE \bfh(Y^{(1)})}
\newcommand{\Ehoo}{\bbE \bfh^{(1)}(Y^{(1)})}
\newcommand{\Ehot}{\bbE \bfh^{(2)}(Y^{(1)})}
\newcommand{\Ehtt}{\bbE \bfh^{(2)}(Y^{(2)})}
\newcommand{\Ezo}{\bbE (Z_l^{(1)})}
\newcommand{\Ezt}{\bbE (Z_l^{(2)})}

% Estimators
\newcommand{\hto}{(\widehat{\btheta}_{1,{\rm ml}})_{n}}
\newcommand{\htto}{(\widehat{\btheta}_{2,{\rm ml}})_{n}}
\newcommand{\httm}{(\widehat{\btheta}_{2,{\rm ml}})_{m}}
\newcommand{\htt}{(\widehat{\btheta}_{2,{\rm ml}})_{n+m}}

\newcommand{\BXn}{\Bar \bX_{1:n}}
\newcommand{\BXm}{\Bar \bX_{n+1:n+m}}
\newcommand{\BXnm}{\Bar \bX_{1:n+m}}
